From Deferral to Learning: Online In-Context Knowledge Distillation for LLM Cascades

Standard LLM cascades improve efficiency by deferring difficult queries from weak to strong models. However, these systems are typically static: when faced with repeated or semantically similar queries, they redundantly consult the expensive model, failing to adapt during inference. To address this, we propose Inter-Cascade, an online, interactive framework that transforms the strong model from a temporary helper into a long-term teacher. In our approach, when the strong model resolves a deferred query, it generates a generalized, reusable problem-solving strategy. These strategies are stored in a dynamic repository and retrieved via similarity matching to augment the weak model's context for future queries. This enables the weak model to learn on the job without expensive parameter fine-tuning. We theoretically show that this mechanism improves the weak model's confidence calibration. Empirically, Inter-Cascade outperforms standard cascades on multiple benchmarks, improving weak model and overall system accuracy by up to 33.06 percent and 6.35 percent, while reducing strong model calls by up to 48.05 percent and saving fee by up to 49.63 percent. Inter-Cascade demonstrates effective in-context knowledge transfer between LLMs and provides a general, scalable framework applicable to both open-source and API-based LLMs.

==> 1_intro.tex <==
\section{Introduction}\label{sec: intorduction}

% Large Language Models (LLMs) demonstrate remarkable performance across a wide range of generation and reasoning tasks. 

% LLMs with stronger performance are generally larger in size, and the converse holds as well~\citep{kaplan2020scalinglawsneurallanguage}. Larger models often achieve better performance on more challenging tasks but are correspondingly more expensive.

% Depending on their expected workload, cost-sensitive users may wish to use \emph{weaker} (and cheaper) models that 
% suffice for simple queries and reserve the use of \emph{stronger} (and expensive) models for more complex queries.

%  In a prototypical example, a weaker model may run on a mobile device such as a phone while a stronger model may run in a cloud-based server owned by another service: the cost of the stronger model can include latency, monetary charges, or both. 
% Since accuracy alone is not the only performance metric of interest, practical deployment scenarios require balancing multiple objectives including efficiency, latency, reliability, and network resource usage~\citep{zhou2024large,khatun2024truthevaldatasetevaluatellm,gundla2025multi,yan2025we,zhou2024large}.

Large Language Models (LLMs) demonstrate strong performance across a wide range of generation and reasoning tasks. Models with stronger performance are generally larger~\citep{kaplan2020scalinglawsneurallanguage} and thus more expensive to run.
Depending on their workload, cost-sensitive users may prefer \emph{weaker} (cheaper) models for routine queries and reserve \emph{stronger} (expensive) models for complex ones.
In a prototypical example, a weaker model may run on a mobile device such as a phone while a stronger model may run in a cloud-based server owned by another service: the cost of the stronger model can include latency, monetary charges, or both.  Accordingly, practical deployments must balance accuracy with efficiency, latency, reliability, and network resource usage~\citep{zhou2024large,khatun2024truthevaldatasetevaluatellm,gundla2025multi,yan2025we,zhou2024large}.


The \textit{LLM Cascade} has emerged as a widespread LLM paradigm in which weaker models handle routine queries and \textit{defer} uncertain cases to stronger models in a sequential order~\citep{chen_frugalgpt_2023}. Deferral depends on a \textit{deferral function}, typically estimates a confidence score that decides when to send queries to the strong model. 
The current approach focuses on improving this deferral decision by training or adjusting the threshold for the confidence score to decide when to defer~\citep{shen_learning_2024,rayan_learning_2025,ong_routellm_2024,zellinger_cost-saving_2025,zellinger_rational_2025,xia_which_2024,nie_online_2024,jung2024trustescalatellmjudges}.
%Existing works have largely focused on improving the \textit{deferral function}, i.e., learning or designing mechanisms that reflect model confidence of a query and decide when to escalate this query to the stronger model (e.g.,~\cn).
% The LLM Cascade methods reduce the usage of strong LLM and requires calibration methods for the confidence~\citep{jung2024trustescalatellmjudges}. 
The strong model, weak model, and deferral function are optimized prior to deployment. After training, the system follows the same pipeline for any incoming query, which means processing is not adaptive to the workflow during inference/deployment. A static LLM Cascade pipeline would result in a substantial waste of tokens. 

NVIDIA’s recent position paper~\citep{belcak2025small} shows that many LLM applications repeatedly perform a small set of specialized tasks with only modest variations. 
%
There are various of scenarios that contain inherently similarities. For instance, datasets like GSM-Plus~\citep{li_gsm-plus_2024}, an extension of a math problem dataset GSM8K~\citep{cobbe_training_2021-1}, contains eight variants for each problem. Identical questions are repeatedly asked: e.g., “Which is larger, 9.9 or 9.11?” Users were once eager to keep asking this question to any newly released LLM
%as a quick test of intelligence
~\citep{korzhov_stop_2023,schnabel_stop_2024,junco_every_2025}.
%
However, current LLM Cascade methods do not take this ``similarity phenomenon'' into consideration. As a result, a large amount of tokens are wasted because of repeated or similar queries.
%
If a weak models consistently fails on similar or recurring problems, the system must repeatedly consult the strong model each time, which is wasteful/costly.
% When a weak model consistently fails on similar or recurring type of hard problems, the cascade system repeatedly consults the strong model, paying the full cost each time. This issue not only wastes resources but also increases latency if stronger model is deployed on remote cloud or accessed via API.
%
The non-interactive nature of traditional LLM cascades, where weak models can only offload, prevents them from leveraging feedback from stronger models' capabilities during generation/inference. Furthermore, fine-tuning weaker models to overcome such failures is expensive and sometimes impractical: fine-tuning requires substantial memory (e.g., finetune Qwen3-235B requires 130 GB VRAM for LoRA or 2560 GB for full-parameter fine-tuning ~\citep{yang2025qwen3technicalreport}) and must re-train again when distributions shift. For API-based models, fine-tuning may not even be available.

%In a sense, current LLM Cascades are inherently ``nonadaptive'', unable to adapt to the actual query stream. 
To take advantage of this phenomenon, in this paper we improve current ``static'' LLM Cascade by developing a new online adaptation method to assist the weaker model in dynamically balancing cost and accuracy. 
%maintaining confidence calibration~\cn they are inherently passive. Once the LLM Cascade is deployed, the deferral rule remains fixed, and the stronger models act only as backup helpers without influencing the weaker models in the long term. 
Our key insight is to exploit input similarity so the strong model can help the weaker one adapt and handle similar queries locally. The essence of the approach is to let the weaker model learn from the stronger model online: the weaker model can build a ``crib sheet'' using prior queries to do prompt engineering at the input that will guide the weaker model to the correct solution locally. 

% As an example of the concept, let us consider scenarios that have
% %Its non-interactive nature leads to inefficiencies for a lot of practical scenarios. In daily applications, queries often form 
% clusters of similar or even identical problems.


Our approach is influenced by in-context learning 
%Alternative approaches such as in-context learning
(ICL)~\citep{dong2024surveyincontextlearning} or few-shot prompting~\citep{parnami2022learningexamplessummaryapproaches}, which can  partially alleviate this limitation. In those approaches, by carefully selecting demonstrations or instructions one can enhance the reasoning capacity of weaker models without retraining. 
%Transformer-based models are inherently flexible in following instructions and adapting to context~\citep{sander2024transformersperformincontextautoregressive}. 
However, existing ICL and few-shot methods often rely on manual prompt design or retrieval from either fixed or manually updated database, making them inflexible as query distributions evolve. Our approach is related to Retrieval-Augmented Generation(RAG)~\citep{lewis_retrieval-augmented_2021}, in which a database is used for assisting the generation of answer. However, the databases in RAG studies are either built with engagement of human~\citep{edge_local_2025,chen2025comrag,shi2024eragent} or updated from single LLM dialogue history for personalization usage~\citep{zhang2025dh,mo2025conversational}, while in our approach, the knowledge corpus are extracted from an extra stronger LLM without any human intervention. The goal in this work is to develop a framework that enables cascaded LLMs to interact adaptively: the weak model can benefit from \emph{in situ} reasoning generated by the strong model to improve its own performance during real-world query streams. As a metaphor,  the weak model uses the strong model for ``on the job'' training to improve longer-term performance. We further discuss this paradigm's relationship to \textbf{Extended Related Works} with details in the Appendix~\ref{sec: related work}.

\noindent \textbf{Primary contributions.}
We improve on existing LLM Cascade approaches. \textbf{(1)} We propose a new framework, \textit{Inter-Cascade}, for online and interactive LLM Cascades in which the strong model serves as both a backup helper and longer-term teacher. The strong model can both answer difficult queries and provide feedback that can be reused by the weak model to generalize problem-solving \emph{strategies} for future queries. These strategies are stored in a local database which the weak model uses as an auxiliary input: its performance is improved on similar future queries by leveraging the strategies generated from the strong model. In this way the strong LLM ``teaches'' the the weak LLM how to resolve these queries on its own. We think of this approach as a kind of \emph{in-context knowledge distillation} approach to LLM Cascade using similarity-based memory. \textbf{(2)} We propose a theoretical model and show that without changing the deferral rule, adding strategies helps the weak LLM's confidence score better approximate its probability of correctness. This shows that using strategies can provably guarantee the higher accuracy of the overall system. \textbf{(3)} We compare to standard LLM Cascade and show that Inter-Cascade improves the weak LLM accuracy by up to 33.06 absolute percentage points and the overall system by up to 5.53 absolute percentage points, while reducing the usage of strong models by up to 48.05\% relative reduction, This can reduce the corresponding fees by up to 49.63\% relative reduction with the same guarantee of risk tolerance and error level over all benchmarks. Crucially, our framework is general and modular: it applies to both API-only models and open-source models, and can be combined with any deferral function or any number of LLMs in cascade. We make the full implementation of Inter-Cascade under an open source license.

%\yw{temporarily commented the paragraph for section schedules}
%Section~\ref{sec: formulation} starts from introducing the formulation of standard LLM Cascade. Then we pick up a success-rate guaranteed LLM Cascade as the baseline of our work and describe the calibration method of confidence threshold we are going to use in our work. And then we extend the passive LLM Cascade diagram to our Inter-Cascade and prove that the adding strategy to weak model ensure a tighter bound on success rate. In section~\ref{sec: experiments}, we conduct experiments from multiple perspective to show that Inter-Cascade achieves higher accuracy while pay less on the use of strong model. We differentiate our Inter-Cascade with other similar frameworks or LLM-boosting methods in Section~\ref{sec: related work}.
% Our contributions in this work are listed as follows:\yw{need revise}
% \begin{enumerate}

%     \item Framework design. To address the inefficiencies of passive cascades, we introduce an interactive pipeline where the strong model serves as both a backup and a teacher, generating reusable knowledge for future queries.
%     \item Theoretically show that  strategy imporve the performance
%     \item Empirical validation. We demonstrate that our approach significantly outperforms existing LLM cascade baselines in both efficiency and reliability. We release our pipeline as open-source, highlighting its scalability and generality to multiple LLMs, routers, and cascade depths.
% \end{enumerate}

% Reasoning tasks inherently require multi‐step inference, significantly increasing computational complexity and resource consumption. In high‐stakes domains, such as healthcare, legal analysis, and scientific research, these reasoning subproblems are unavoidable, and as LLM usage proliferates, a single query can encompass thousands of such subproblems, driving inference time and cost to prohibitive levels (ref). At the same time, ensuring answer correctness is critical: when the model is uncertain, it should notify the user rather than risk a misleading response. (may add some refs here) To address both concerns—reducing LLM computation and expense while simultaneously improving answer accuracy and signaling uncertainty, we refine the framework of (ref) by introducing an in‐context learning feedback loop.

% (ref ...) introduces a way of selective evaluation framework, provably guarantees agreement between the LLM evaluation and human judgment. The framework begins with a Selective Evaluation paradigm: an LLM judge only issues a preference when its confidence—calibrated on a small validation set—exceeds a predefined threshold, otherwise it abstains. This guarantees that any retained judgments meet a user‐specified level of human agreement. To minimize cost, the authors introduce Cascaded Selective Evaluation, where judgments first pass through a smaller, less expensive LLM; only instances with low confidence “escalate” to a larger, costlier model. By carefully calibrating confidence estimates and thresholds at each stage, the cascade ensures that all final judgments maintain the desired human‐agreement guarantee while reducing reliance on high‐cost models.

% \yw{integrate this part to (d)}We adopt a similar framework for reducing LLM computation and expense—without focusing on guaranteeing human agreement in the LLM’s evaluations. Our refinement introduces a feedback loop from the strong LLM to the weak LLM. Specifically, when the strong LLM is tasked with solving a problem, it returns not only the solution but also an indicative strategy that captures its reasoning process. We store these strategies in a reference document. Then, when the weak LLM encounters a new problem, we retrieve similar problems from this document and append the corresponding strong‐LLM strategies to the prompt, effectively teaching the weak LLM how to approach the new problem. By leveraging the strong LLM’s outputs in this feedback loop, the weak LLM can solve more questions on its own, reducing the number of calls to the strong LLM and thereby saving both computation and cost.

% By calibrating a confidence threshold $\tau_1,\tau_2$ for the weak and strong LLM, respectively—analogous to the Selective Evaluation paradigm in (ref)—we ensure
% \[
% \Pr\bigl(\text{weak‐LLM output is correct} \mid \text{confidence} \ge \tau\bigr) \;\ge\; 1 - \varepsilon\,,
% \]
% so any instance with confidence below $\tau_1$ defers to the strong LLM. Likewise, we choose a threshold $\tau_2$ for the strong LLM such that
% discarding any low‐confidence outputs to preserve the strategy document’s integrity. Together, these thresholds bound the overall error rate for both weak LLM outputs and stored strategies, while minimizing reliance on costly strong‐LLM calls.





==> abstract.tex <==
\begin{abstract}
    Large Language Models (LLMs) vary widely in their capabilities, with larger models often having better performance but higher cost: choosing an LLM model often involves trading off performance and cost. The \textit{LLM Cascade} is a paradigm that \textit{defers} difficult queries from weak/cheap to strong/expensive models. This approach is nonadaptive: the deferral decision\ywadd{ rule} is trained\ywadd{ or derived by algorithms} offline.
    %
    When confronted with similar or repeated queries, the LLM Cascade may then repeatedly consult the expensive model and incur higher cost.
    %
    %
    To improve the cascading efficiency, we propose \textit{Inter-Cascade}, an online and interactive LLM Cascade that extends the role of strong model from a backup helper to a long-term teacher. 
    %
    %
    In our system, when a strong model resolves a difficult query, it also distills its solution into a generalized, reusable problem-solving strategy that boosts the weak model on subsequent queries. 
    %
    %
    %This approach enables
    Adding strategies to queries enables the weak model to dynamically improve its performance over time, avoiding computationally and time-intensive fine-tuning.
    %
    %
    Empirically, compared with standard LLM Cascade baselines across multiple benchmarks, the Inter-Cascade significantly improves the accuracy of the weak model (by up to 33.06 absolute percentage points) and the overall system (by up to 5.53 absolute percentage points), while reducing the calls to strong models (by up to 48.05\% relative reduction) and saving the corresponding fees (by up to 49.63\% relative reduction). 
    %
    Inter-Cascade demonstrates the effective in-context knowledge transfer between LLMs, and provides a general, scalable framework applicable to both open-source and API-based LLMs.

\end{abstract}


==> make_title.tex <==


\maketitle

==> title.tex <==



\title{Not only a helper, but also a teacher: Interactive LLM Cascade}

%other candidate:
%Collaboration with feedback: Interactive Learning to defer for LLMs collaboration


% Authors must not appear in the submitted version. They should be hidden
% as long as the \iclrfinalcopy macro remains commented out below.
% Non-anonymous submissions will be rejected without review.

% Custom command for symbols
\newcommand{\affilone}{\textsuperscript{\dag}}
\newcommand{\affiltwo}{\textsuperscript{\ddag}}
\newcommand{\affilthree}{\textsuperscript{\S}}
% \newcommand{\equal}{\textsuperscript{\P}}
\newcommand{\equalcontri}{\textsuperscript{=}}
\newcommand{\corrauth}{\textsuperscript{*}}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}%
  \textsuperscript{}%
  \footnotetext[0]{#1}%
  \endgroup
}


\author{%
  Yu Wu\affilthree\equalcontri, 
  Shuo Wu\affiltwo\equalcontri, 
  Ye Tao\affilthree\equalcontri, 
  Yansong Li\affiltwo, 
  Anand D. Sarwate\affilthree\corrauth \\
  \affilthree Rutgers University,
  \affiltwo University of Illinois Chicago
}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
%\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.


% Authors must not appear in the submitted version. They should be hidden
% as long as the \iclrfinalcopy macro remains commented out below.
% Non-anonymous submissions will be rejected without review.

